DiffuStereo: High Quality Human Reconstruction via Diffusion-based Stereo Using Sparse Cameras

We propose DiffuStereo, a novel system using only sparse cameras (8 in this work) for high-quality 3D human reconstruction. At its core is a novel diffusion-based stereo module, which introduces diffusion models, a type of powerful generative models, into the iterative stereo matching network. To this end, we design a new diffusion kernel and additional stereo constraints to facilitate stereo matching and depth estimation in the network. We further present a multi-level stereo network architecture to handle high-resolution (up to 4k) inputs without requiring unaffordable memory footprint. Given a set of sparse-view color images of a human, the proposed multi-level diffusion-based stereo network can produce highly accurate depth maps, which are then converted into a high-quality 3D human model through an efficient multi-view fusion strategy. Overall, our method enables automatic reconstruction of human models with quality on par to high-end dense-view camera rigs, and this is achieved using a much more light-weight hardware setup. Experiments show that our method outperforms state-of-the-art methods by a large margin both qualitatively and quantitatively.

==> section_intro-old.tex <==
\section{Introduction}
High quality 3D human reconstruction is the key to large number of applications ranging from telecommunications, education, entertainment, and so on. High-end systems~\cite{bradley2008markerless,gall2009motion,liu2009point,brox2009combined,liu2011markerless,pons2017clothcap} based on dense camera rigs (up to 100 cameras~\cite{collet2015high}) and custom-designed lighting conditions~\cite{guo2019relightables} can achieve high-quality reconstruction, but the sophisticated setup limits their deployment in practice. 
Recently, researchers have proposed to employ neural implicit functions to reconstruct 3D humans from single-view RGB~\cite{saito2019pifu,saito2020pifuhd}, sparse-view RGB~\cite{Huang_2018_ECCV,zheng2021deepmulticap} or sparse-view RGBD inputs~\cite{yu2021function4d}. Thanks to the representation power of deep implicit functions, impressive results have been demonstrated and inspired many follow-up works~\cite{zheng2021pamir,Huang2020ARCH,he2021arch++,li2021posefusion}. 


% And the underlying technique, volumetric capture, is
% a challenging and long-standing problem in both computer
% vision and computer graphics due to the complex shapes,
% fast motions, and changing topologies that need to
% be faithfully reconstructed. Although high-end volumetric
% capture systems~\cite{} based on dense camera
% rigs (up to 100 cameras~\cite{}) and custom-designed lighting
% conditions~\cite{} can achieve high-quality reconstruction,
% they all suffer from complicated system setups and are limited to professional studio usage.](mainly copied from function4D) Recently, the neural implicit representation has been proposed to reconstruct human under sparse views. However, the geometry quality of existing methods is still lower than the traditional dense camera rigs. PIFuHD, DeepMultiCap utilize the predicted normal map and the multi-level network structure to recover the geometry details. But it is difficult to ensure the consistency of predicted normal map under sparse views. Function4D achieves real-time volumetric capture with 3 RGB-D cameras. But the quality of reconstruction is limited by the resolution of depth sensors. 

Despite the rapid development in sparse-view human reconstruction, existing methods are still incapable to generate results comparable to dense multi-view camera rigs.
Dense-view systems explicitly utilize stereo matching to establish pixel correspondences among different views, which is essential to compute accurate 3D surface locations. In contrast, current learning-based sparse-view methods heavily rely on the appearance cues and other high-level semantics in each individual image to infer the geometry, ignoring the hints provided by cross-view pixel correspondences.  
% This is mainly because dense-view reconstruction methods explicitly utilize stereo matching to compute pixel correspondences among different views , while sparse-view methods heavily rely on the neural network to .... 
% StereoPIFu~\cite{yang2021stereopifu} pioneered in combining stereo matching with implicit reconstruction to improve reconstruction accuracy through constructing a 3D cost volume, but such a method comes at a high computational cost and limits the possible operating resolution. 
To ensure both accuracy and high-quality reconstruction, it is necessary introduce stereo matching methods into sparse-view reconstruction systems.
% Recently, stereo-PIFu shows that combining stereo and implicit reconstruction can further improve the accuracy of geometry. 
% To ensure both accuracy and high-quality reconstruction, it is necessary introduce stereo matching methods into sparse view systems.
StereoPIFu~\cite{yang2021stereopifu} pioneered in combining stereo and implicit reconstruction to improve the accuracy of geometry via constructing a 3D cost volume, but such a scheme comes at a high computational cost and limits the possible operating resolution. 


To make stereo matching more efficient, RAFT-stereo~\cite{lipson2021raftstereo} proposed an iterative stereo matching method and perform convolution in 2D domain. 
% However, the predominant stereo approach mostly build a 3D cost volume by enumerating integer disparities and use 3D convolutional neural networks to filter it. Such processing way comes at a high computational cost and limits the possible operating resolution. Raft-stereo proposes an iterative and efficient stereo matching by replacing 3D convolution with 2D convolution. 
But the quality of Raft-stereo is still limited by the discrete per-pixel cost volume and the number of iterations for refinement. Another challenge for human stereo is the sparse camera setting since existing binocular stereo usually assumes two views are close. Both the flow and the occlusion region between two views are relatively small. However, these assumptions are invalid under the sparse camera settings. The flow estimation easily fall into the local minimum and the large occlusion region can not be neglected.

Very recently, diffusion model has been proposed to synthesis high-quality and photo-realistic images~\cite{}. The powerful generative ability of diffusion model even beats GAN~\cite{}. The key insight of diffusion model is to learn the gradient of data distribution. As mentioned in ~\cite{}, the diffusion process can be regarded as learning to solve a continuous stochastic differential equations. Meanwhile, traditional stereo methods based on continuous variational approach~\cite{} also solve the differential equations to overcome the discretization limitations and estimate the sub-pixel level flow. Such similarity inspires us to combine the continuity of diffusion 
model with existing learning-based discrete stereo to achieve high quality human depth estimation. 

In this paper, we propose HQCap to solve the challenging problem for high quality human volumetric performance under sparse views. The insight of our system is to combine the stereo matching with diffusion process to further refine the geometry reconstructed by existing implicit-based method. In particular, we first adopt DoubleField to reconstruct a coarse human mesh and obtain the coarse depth maps of each view by rendering it. To deal with the challenge of stereo for sparse views, we further utilize the coarse depth maps 
% to avoid local optimum 
by transforming it as the initial flow and compute a mask for most occlusion areas. Then the key problem is to estimate the high quality human depth maps by binocular stereo for each two neighboring views. There are two challenges in this task:  1)  High quality and accuracy of depth estimation. To overcome the discretization problem and achieve sub-pixel level flow prediction, we propose a continuous diffusion model to iteratively refine the coarse flow. \srz{more explanations about diffusion process.} We also condition the diffusion network with several features to ensure stereo consistency and add epipolar constraint to the predicted flow. 2) Memory issues for high-resolution images. Since we focus on the high quality of flow estimation, we further design a multi-level network structure to tackle with the memory issues for high-resolution images. Following PIFuHD~\cite{}, our network contains two level: the global level which extracts human semantic feature from downsampled image, the diffusion level which introduces the global feature into the proposed diffusion stereo network and iteratively refine flow. The multi-level structure enables the network trained in a patch-based way and thus resolve the memory issues caused by high-resolution images.

Moreover, we propose a light-weight multi-view hybrid fusion to deal with calibration error on real-world data and fix the occlusion region in stereo matching. Our fusion method  further align the refined depth point cloud of each view and the coarse human model by non-rigid ICP. Then we select the points in the coarse mesh to fix the occlusion part and reconstruct the final model.
In comparison with existing approaches for human volumetric performance capture, our method can reconstruct high quality human model using only 8 passive cameras. The quality of our geometry reconstruction in visible region is even competitive with the ground truth on THuman2.0 dataset. Moreover, our system can reconstruct one high-quality human model in 15s, which is much faster than traditional methods based on dense camera rigs. In summary, our contributions in this work are:

\noindent 1) We propose HQCap, a light-weight and high-quality system for human volumetric capture under sparse multi-views.

\noindent 2) To the best of our knowledge, we are the first one to introduce the diffusion model into stereo and human reconstruction. We propose a novel multi-level diffusion stereo network to achieve accurate and high-quality human depth estimation.

% Since stereo need to estimate the correspondences which can be formulated as flow from one view to another view. 

% Next: raft-stereo use 2D cost volume. higher resolution but still discrete per-pixel matching.

% Next: Diffusion: continuous and powerful

% \srz{Sparse view challenging for stereo. Need DoubleField coarse model!}

% \textbf{Combining diffusion and stereo}. How and Why

% \textbf{Light-weight fusion}. Fast and retain details.

% \textbf{Contribution}
% 1. system
% 2. diffusion
% 3. light-weight fusion
